A Decentralized Multi-Agent Unmanned Aerial System to Search, Pick Up, and Relocate Objects

We present a fully integrated autonomous multi- robot aerial system for finding and collecting moving and static objects with unknown locations. This task addresses multiple relevant problems in search and rescue (SAR) robotics such as multi-agent aerial exploration, object detection and tracking, and aerial gripping. Usually, the community tackles these problems individually but the integration into a working system generates extra complexity which is rarely addressed. We show that this task can be solved reliably using only simple components. Our decentralized system uses accurate global state estimation, reactive collision avoidance, and sweep planning for multi-agent exploration. Objects are detected, tracked, and picked up using blob detection, inverse 3D-projection, Kalman filtering, visual-servoing, and a magnetic gripper. We evaluate the individual components of our system on the real platform. The full system has been deployed successfully in various public demonstrations, field tests, and the Mohamed Bin Zayed International Robotics Challenge 2017 (MBZIRC). Among the contestants we showed reliable performances and reached second place out of 17 in the individual challenge.

==> sections/challenge_description.tex <==
The system is mainly motivated by the third challenge of the \ac{mbzirc} benchmarking competition\footnote{www.mbzirc.com}.
Challenge 3 requires a team of three \acp{mav} equipped with grippers to search, find, pick, and relocate a group of static and moving objects in a $60 \unit{m} \times 90 \unit{m}$ planar arena.
The challenge lasts a maximum of 20 minutes.
The arena has 6 moving and 10 stationary small objects as well as 3 stationary large objects.
The moving objects move at random velocity lower than $5 \unit{km/h}$.
Small objects have a cylindrical shape with diameter $200 \unit{mm}$ and a maximum weight of $500 \unit{g}$.
Large objects have a rectangular shape with dimensions $150 \unit{mm} \times 2000 \unit{mm}$ and a weight not exceeding $2 \unit{kg}$.
In this work we ignore lifting of large objects.
The object color determines the object type and score.
Teams gain points with each successful delivery to the drop container or drop zone.
In the grand challenge the third challenge runs simultaneously to the first and second challenge which introduces additional interaction with other robotic platforms.
\begin{figure}
  \centering
  \includegraphics[width=0.48\textwidth]{figures/arena}
  \caption{\ac{mbzirc} challenge 3: Starting from the \acf{lz} our three \acp{mav} need to collect all objects in the arena and deliver them to the \acf{dz} or drop box.
  The top right image shows our platforms consisting of three identical \ac{asctec} Neo hexacopters equipped with a downward-facing RGB camera, \ac{epm} gripper, VI-sensor, and RTK-GPS receiver.
  The bottom right image shows a successful delivery during a \ac{mbzirc} trial.}
  \label{fig:arena}
\end{figure}

